Survey on Teleoperation Concepts for Automated Vehicles

In parallel with the advancement of Automated Driving (AD) functions, teleoperation has grown in popularity over recent years. By enabling remote operation of automated vehicles, teleoperation can be established as a reliable fallback solution for operational design domain limits and edge cases of AD functions. Over the years, a variety of different teleoperation concepts as to how a human operator can remotely support or substitute an AD function have been proposed in the literature. This paper presents the results of a literature survey on teleoperation concepts for road vehicles. Furthermore, due to the increasing interest within the industry, insights on patents and overall company activities in the field of teleoperation are presented.

==> Tables/overview_table.tex <==
\begin{table}[!htb]
 
\caption{Overview Control Concepts}\label{tab:contrConcepts} \centering 
\begin{tabularx}{0.47\textwidth}{XXXX} 
%header
\toprule
\textbf{Concept}  & \textbf{Publications} & \textbf{Input Devices} \\

\midrule
\multirow{1}{=}{Direct Control}
& \cite{Gnatzig2013ToDSystemDesign, Hofbauer2020telecarla, Schimpe21oss4tod, Jatzkowski2021, 5GCroCoD2p2, Appelqvist2007, Bensoussan1997, Bodell2016, Ross2007, Shen2016, Wu} & Steering W. \& Ped. \\
%& \cite{Gnatzig2013ToDSystemDesign} & Steering W. \& Ped.   \\
%& \cite{Hofbauer2020telecarla} & Steering W. \& Ped.  \\
%& \cite{Schimpe21oss4tod} & Steering W. \& Ped.   \\
%& \cite{Jatzkowski2021} & Steering W. \& Ped.  \\
%& \cite{5GCroCoD2p2} & Steering W. \& Ped.  \\
%& \cite{Appelqvist2007} & Steering W. \& Ped.    \\
%& \cite{Bensoussan1997} & Steering W. \& Ped.    \\
%& \cite{Bodell2016} & Steering W. \& Ped.    \\
%& \cite{Ross2007} & Steering W. \& Ped.    \\
%& \cite{Shen2016} & Steering W. \& Ped.    \\
%& \cite{Wu} & Steering W. \& Ped.    \\

\midrule
\multirow{2}{=}{Shared Control}
& \cite{Schimpe2020steerwithme, Anderson2013, Qiao2021, Saparia21ass4tod, Storms2017sharedControl4oa} & Steering W. \& Ped. \\
& \cite{Schitz2021acc} & ? \\

\midrule
\multirow{1}{=}{Trajectory Guidance}
& \cite{Gnatzig2012trajBasedSharedAutonomy, Hoffmann2022a} & Steering W. \& Ped. \\

\midrule
\multirow{2}{=}{Waypoint Guidance}
& \cite{5GCroCoD2p2, Schitz2021, Jatzkowski2021, Kay1995a} & Mouse \& Keyboard \\
& \cite{Bjornberg2020} & Virtual Joystick \\

\midrule
\multirow{2}{=}{Interactive Path Planning}
& \cite{Hosseini2014a, Schitz2021interactivePathPlanning} & Mouse \& Keyboard \\
& $~$ \\

\midrule
\multirow{2}{=}{Perception Modification}
& \cite{Feiler2021percmod} &  Mouse \& Keyboard \\
& &  \\

\bottomrule
\end{tabularx} 
\end{table}



==> Tables/taxonomy_table.tex <==
\newcolumntype{s}{>{\hsize=.45\hsize}X}

\begin{table}[b]
	
	\caption{Taxonomy}\label{tab:taxonomy} \centering 
	\begin{tabularx}{0.47\textwidth}{sXXX} 
		%header
		\toprule
		\textbf{Term}  & \textbf{Description} \\
		
		\midrule
		\multirow{1}{*}{Remote Monitoring}
		& No interaction. The system is being remotely monitored. \\
		
		\midrule
		\multirow{1}{*}{Remote Driving}
		& The system is being fully under remote control. Direct control, Shared control. SAE L1 and L2. \\
		
		\midrule
		\multirow{1}{*}{Remote Assistance}
		& The system is receiving some level of remote assistance from operator, while still being responsible for driving task. Indirect control modes. SAE L4, L5. \\
		
		\midrule
		\multicolumn{2}{c}{Teleoperation}\\
		
		\bottomrule
 	\end{tabularx} 
\end{table}
